Spatio-Temporal Data Mining: A Survey of Problems and Methods

Large volumes of spatio-temporal data are increasingly collected and studied in diverse domains including, climate science, social sciences, neuroscience, epidemiology, transportation, mobile health, and Earth sciences. Spatio-temporal data differs from relational data for which computational approaches are developed in the data mining community for multiple decades, in that both spatial and temporal attributes are available in addition to the actual measurements/attributes. The presence of these attributes introduces additional challenges that needs to be dealt with. Approaches for mining spatio-temporal data have been studied for over a decade in the data mining community. In this article we present a broad survey of this relatively young field of spatio-temporal data mining. We discuss different types of spatio-temporal data and the relevant data mining questions that arise in the context of analyzing each of these datasets. Based on the nature of the data mining problem studied, we classify literature on spatio-temporal data mining into six major categories: clustering, predictive learning, change detection, frequent pattern mining, anomaly detection, and relationship mining. We discuss the various forms of spatio-temporal data mining problems in each of these categories.

==> evaluation.tex <==

\section{Evaluation}

Results generated using spatio-temporal data mining approaches needs to be thoroughly evaluated to ensure that they are not due to previously known properties of the underlying data. Extensive work was done in designing evaluation strategies for classification, clustering, and pattern mining on relational data. Many of these evaluation strategies were adopted for similar problems defined over time series data and spatial data. Designing evaluation strategies for problems defined over spatio-temporal data sets is non-trivial due two reasons: i) problems themselves are relatively more complex, ii) both temporal and spatial properties of the data have to be dealt with.

$\bullet$ {\color{red} Dealing with spuriousness due to  autocorrelation}

$\bullet$ {\color{red} Recent approaches for diffrent problems}



